Optimal Sequential Task Assignment and Path Finding for Multi-Agent Robotic Assembly Planning

We study the problem of sequential task assignment and collision-free routing for large teams of robots in applications with inter-task precedence constraints (e.g., task $A$ and task $B$ must both be completed before task $C$ may begin). Such problems commonly occur in assembly planning for robotic manufacturing applications, in which sub-assemblies must be completed before they can be combined to form the final product. We propose a hierarchical algorithm for computing makespan-optimal solutions to the problem. The algorithm is evaluated on a set of randomly generated problem instances where robots must transport objects between stations in a "factory "grid world environment. In addition, we demonstrate in high-fidelity simulation that the output of our algorithm can be used to generate collision-free trajectories for non-holonomic differential-drive robots.

==> graphics/simple_project_schedule_graph.tex <==
      % \graph [grow right sep] {
      %   {
      %     o1 [ObjectNode,as=O1],
      %     r1 [RobotNode, as=R1] -> go1 [ActionNode, as=GO]
      %   } -> {
      %     collect1 [ActionNode, as=COLLECT] -> 
      %       carry1 [ActionNode, as=CARRY] -> 
      %         deposit1 [ActionNode, as=DEPOSIT] 
      %   } -> {
      %     r1e [RobotTerminalNode, as=R1],
      %     {
      %       op1 [OpNode, as=O1] -> 
      %         o3 [ObjectNode, as=O3]} -> {
      %           collect3 [ActionNode, as=COLLECT] -> 
      %             carry3 [ActionNode, as=CARRY] -> 
      %               deposit3 [ActionNode, as=DEPOSIT] ->  {
      %                 op3 [OpNode, as=OP3],
      %                 r2e [RobotTerminalNode, as=R2]
      %       },
      %     },
      %   },
      %   {
      %     o2 [ObjectNode,as=O1], 
      %     r2 [RobotNode, as=R2] -> go2 [ActionNode, as=GO]
      %   } -> {
      %     collect2 [ActionNode, as=COLLECT] -> carry2 [ActionNode, as=CARRY] -> deposit2 [ActionNode, as=DEPOSIT] -> {
      %       op1,
      %       go3 [ActionNode, as=GO] -> collect3
      %     }
      %   }
      % };

==> results/assignment_milp_runtime_factor.tex <==
\begin{tikzpicture}[scale={0.7}]
\centering
\pgfplotsset{set layers=standard,cell picture=true}

\begin{groupplot}[group style={group name={myPlots}, group size={6 by 1}, xlabels at={edge bottom}, xticklabels at={edge bottom}, vertical sep={0pt}, horizontal sep={2pt}}, boxplot, boxplot/draw direction={y}, ymode={normal}, footnotesize, width={\plotarraywidth}, height={\plotarrayheight}, xmin={0}, xmax={4}, ymin={-10}, ymax={10}, xtick={10,20,30}, xticklabels={10,20,30}, tickpos={left}, ytick={0.1,1.0,10.0,100.0}, yticklabels={}, ylabel shift={0pt}, ytick align={outside}, xtick align={outside}, legend entries={$n = 10$,$n = 20$,$n = 30$}, legend cell align={left}, legend to name={grouplegend}, legend style={draw={black}, fill={white}, xshift={2pt}, inner sep={1pt}, yshift={0pt}, font={\plotarrayfontsize}}, legend pos={north west}]
    \nextgroupplot[xlabel={$m = 10$}, ylabel={relative solver time}, yticklabels={0.1,1.0,10.0,100.0}]
    \addlegendimage{no markers,blue}
    \addlegendimage{no markers,red}
    \addlegendimage{no markers,brown}
    \addlegendimage{no markers,black}

    \addplot+[boxplot]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            3.272594589361159  \\
            1.9806484823105495  \\
            2.878629785096147  \\
            1.102571055356142  \\
            4.60540286014059  \\
            0.6137248043158242  \\
            5.439726618026151  \\
            1.0366798277592693  \\
            5.283332017400086  \\
            2.680434982251498  \\
            3.8341827316850225  \\
            2.563384178742189  \\
            4.421063091443195  \\
            1.3285640998962147  \\
            4.689443871929326  \\
            1.9843799050358688  \\
        }
        ;
    \addplot+[boxplot]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            3.405455223116805  \\
            5.140720579810653  \\
            3.7288924433569965  \\
            5.425933614034411  \\
            5.44781732430009  \\
            3.576953250018501  \\
            6.586423733411457  \\
            2.1044378037193567  \\
            3.2263440645670287  \\
            1.6882538459985454  \\
            3.5591839401140613  \\
            6.117021181680507  \\
            4.434140564092571  \\
            6.542799056032624  \\
            4.282838263969206  \\
            4.70940334218596  \\
        }
        ;
    \addplot+[boxplot]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            6.966132736116592  \\
            6.747103396283092  \\
            7.3290511400341005  \\
            3.647138703434393  \\
            6.036783723124458  \\
            3.1367306689924677  \\
            4.854127730159208  \\
            7.905802498089717  \\
            6.798199535161917  \\
            3.639874531317779  \\
            13.682397756322842  \\
            5.601479813618428  \\
            6.860508925037952  \\
            5.647637061736637  \\
            7.387500403215937  \\
            7.173097631271774  \\
        }
        ;
    \nextgroupplot[xlabel={$m = 20$}, ymajorticks={false}, yminorticks={false}]
    \addplot+[boxplot]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            15.73616336531403  \\
            2.1081509677617163  \\
            4.007070595934415  \\
            3.2197569284214866  \\
            4.394101141600092  \\
            6.596997973360897  \\
            2.368541320835144  \\
            5.867349308248067  \\
            3.647697730789015  \\
            0.22794715150076816  \\
            8.19863219214193  \\
            10.476641723741007  \\
            7.973257390066529  \\
            2.8400019969723176  \\
            2.3963250954638786  \\
            5.056329640410742  \\
        }
        ;
    \addplot+[boxplot]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            4.835455851928887  \\
            4.331586754127084  \\
            4.891915139558232  \\
            3.2312963911764294  \\
            5.02705255753876  \\
            2.636504860611019  \\
            4.057719195244031  \\
            4.395883473009922  \\
            5.8053136197210256  \\
            4.716943324758159  \\
            4.716452151975649  \\
            2.2674519875756944  \\
            5.130807806877803  \\
            6.7197356524718845  \\
            4.832384528579694  \\
            2.414362745086602  \\
        }
        ;
    \addplot+[boxplot]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            4.759351032154148  \\
            5.0077734941444385  \\
            6.449418531145416  \\
            4.747624672360306  \\
            4.246801237927063  \\
            5.485450156297806  \\
            6.729571703688217  \\
            4.899432655233409  \\
            4.125554098345745  \\
            5.579573870152816  \\
            5.571409685042021  \\
            3.688209661842582  \\
            4.730886425801933  \\
            4.892917137667024  \\
            7.014136027021108  \\
            4.2868494917042295  \\
        }
        ;
    \nextgroupplot[xlabel={$m = 30$}, ymajorticks={false}, yminorticks={false}]
    \addplot+[boxplot]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.5730715384627357  \\
            1.1564237574091305  \\
            5.614177270709202  \\
            2.7970744908502527  \\
            0.9169820731570578  \\
            18.647336055144827  \\
            18.449031199759364  \\
            -0.9413209779127474  \\
            0.2942518911967473  \\
            4.2751404669041335  \\
            83.64752438199486  \\
            -0.6192235061895834  \\
            0.5536902984812134  \\
            -0.017978242626120213  \\
        }
        ;
    \addplot+[boxplot]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            4.415145392626314  \\
            6.261663497672966  \\
            4.588879048336005  \\
            5.302487586399223  \\
            4.613698485722279  \\
            4.669503102284231  \\
            7.707418635561167  \\
            3.3847836320958122  \\
            5.3173499728742515  \\
            4.09467690870355  \\
            3.1787906206271863  \\
            6.592578566715313  \\
            6.312884424954774  \\
            3.0233863501774114  \\
            4.937433275933161  \\
            5.048799924874278  \\
        }
        ;
    \addplot+[boxplot]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            4.682685488639835  \\
            3.103384083220508  \\
            4.899744598846621  \\
            2.735653828153321  \\
            5.117534029159146  \\
            7.732793138071546  \\
            3.680229807858434  \\
            4.048007592852952  \\
            3.128840167256272  \\
            5.258759230965465  \\
            3.9093532014989716  \\
            3.983428913421287  \\
            3.953888005767662  \\
            6.828632596988629  \\
            4.481310457292225  \\
            3.7944188887472188  \\
        }
        ;
    \nextgroupplot[xlabel={$m = 40$}, ymajorticks={false}, yminorticks={false}]
    \addplot+[boxplot]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            2.4894636018833642  \\
            -0.20928069716142123  \\
            -0.0413433483362174  \\
        }
        ;
    \addplot+[boxplot]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            2.221122288913333  \\
            2.6094557087387935  \\
            0.23690347269085246  \\
            3.064114560131393  \\
            5.497982008272521  \\
            3.9530243220336145  \\
            2.6142001584006285  \\
            2.277554003339283  \\
            2.5581811233635787  \\
            9.191574296849426  \\
            2.5851555408577997  \\
            3.4802848525028893  \\
            0.31861282281203124  \\
            1.9717810848714066  \\
            2.389463627728309  \\
            1.4200705604748913  \\
        }
        ;
    \addplot+[boxplot]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            11.023501357506893  \\
            6.191244277078964  \\
            5.344534399560955  \\
            3.3281783768228568  \\
            3.2200915753863835  \\
            2.8728514234905025  \\
            3.454674468490244  \\
            2.9797176597655475  \\
            3.345839198131742  \\
            5.446122417608547  \\
            3.7801498174101074  \\
            4.535437296841163  \\
            3.204754663350193  \\
            3.5070374507036757  \\
            3.933771756475377  \\
            1.7568542655617867  \\
        }
        ;
    \nextgroupplot[xlabel={$m = 50$}, ymajorticks={false}, yminorticks={false}]
    \addplot+[boxplot]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            -0.0698315549145554  \\
        }
        ;
    \addplot+[boxplot]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            4.028035133306946  \\
            10.722985365176061  \\
            7.491134318640973  \\
            1.5705235191399256  \\
            25.63194682215373  \\
            0.45930212700643525  \\
            1.2164825402177006  \\
            2.16022582607278  \\
            -0.0999189839955488  \\
            4.27974481510224  \\
            -0.481981136972468  \\
            3.437643251448733  \\
            3.305015302678034  \\
            41.04344771849799  \\
            15.019048142237528  \\
            8.509404586597611  \\
        }
        ;
    \addplot+[boxplot]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            2.4625319554101615  \\
            3.0130915558647913  \\
            2.8096175891618635  \\
            3.346558616689034  \\
            8.284739996655002  \\
            2.6041968119427055  \\
            2.9285971042132544  \\
            5.249416257115796  \\
            2.47097144703969  \\
            1.8523151532514437  \\
            7.434743086226091  \\
            1.3081798438347654  \\
            2.3083538010555134  \\
            7.980175880502687  \\
            0.6356311139443249  \\
            1.972510035341736  \\
        }
        ;
    \nextgroupplot[xlabel={$m = 60$}, ymajorticks={false}, yminorticks={false}]
    \addplot+[boxplot]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.0 \\
        }
        ;
    \addplot+[boxplot]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            23.879808297553517  \\
            -0.13097589118551675  \\
            6.488497519612959  \\
            18.057296499939607  \\
            5.030032760579968  \\
            -0.5595575461949237  \\
            0.46104081454772305  \\
            25.298019666103155  \\
            3.6375836757566193  \\
            24.892960831163904  \\
            -0.38702519726103807  \\
            13.702833562950815  \\
            1.9954450749319075  \\
            4.295611591519805  \\
        }
        ;
    \addplot+[boxplot]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            9.756438298172021  \\
            2.9160448211180023  \\
            1.2362150340851619  \\
            7.345139623568078  \\
            4.900659943180229  \\
            2.704530138836494  \\
            2.9817335987344995  \\
            7.334944815626658  \\
            3.2363310686973326  \\
            9.458673185079851  \\
            3.6667522104302095  \\
            15.23698612554238  \\
            0.7743327561879749  \\
            10.098552366821004  \\
            17.375965259562975  \\
            5.138994356509393  \\
        }
        ;
\end{groupplot}
\node[anchor= north west] (leg) at (myPlots c1r1.north west){\pgfplotslegendfromname{grouplegend}};

\end{tikzpicture}


==> results/single_project/test/low_level_search_without_repair.tex <==
\begin{tikzpicture}[scale={0.7}]
\centering
\pgfplotsset{set layers=standard,cell picture=true}

\begin{groupplot}[group style={group name={myPlots}, group size={6 by 1}, xlabels at={edge bottom}, xticklabels at={edge bottom}, vertical sep={0pt}, horizontal sep={2pt}}, boxplot, boxplot/draw direction={y}, ymode={log}, footnotesize, width={\plotarraywidth}, height={\plotarrayheight}, xmin={0}, xmax={5}, ymin={0.007}, ymax={120}, xtick={10,20,30,40}, xticklabels={10,20,30,40}, tickpos={left}, ytick={0.1,1.0,10.0,100.0}, yticklabels={}, ylabel shift={0pt}, ytick align={outside}, xtick align={outside}]
    \nextgroupplot[xlabel={$m = 10$}, ylabel={time (s)}, yticklabels={0.1,1.0,10.0,100.0}, legend style={draw={none}, fill={white}, xshift={2pt}, yshift={0pt}}, legend pos={north west}]
    \addlegendentry[] {$n = 10$}
    \addlegendentry[] {$n = 20$}
    \addlegendentry[] {$n = 30$}
    \addlegendentry[] {$n = 40$}
    \addlegendimage{mark=*,blue}
    \addlegendimage{mark=*,red}
    \addlegendimage{mark=*,brown}
    \addlegendimage{mark=*,black}

    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.187375417  \\
            0.025500617  \\
            0.015484772  \\
            0.015193346  \\
            0.023005051  \\
            0.023087134  \\
            0.02921947  \\
            0.025804128  \\
            0.024857153  \\
            0.013482373  \\
            0.016895919  \\
            0.029175594  \\
            0.013854146  \\
            0.018176374  \\
            0.025641357  \\
            0.027728509  \\
        }
        ;
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.069536861  \\
            0.06163658  \\
            0.067137013  \\
            0.037564896  \\
            0.054135795  \\
            0.027652065  \\
            0.057545127  \\
            0.050648255  \\
            0.059946934  \\
            0.04074797  \\
            0.030899259  \\
            0.053177729  \\
            0.042518576  \\
            0.050836483  \\
            0.057763364  \\
            0.050457278  \\
        }
        ;
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.08143392  \\
            0.094408913  \\
            0.102619919  \\
            0.073221326  \\
            0.076607729  \\
            0.070595976  \\
            0.100278534  \\
            0.087927087  \\
            0.07884193  \\
            0.064419912  \\
            0.061869379  \\
            0.071676921  \\
            0.06152018  \\
            0.070338489  \\
            0.069408613  \\
            0.062836284  \\
        }
        ;
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.123383468  \\
            0.106442968  \\
            0.099243567  \\
            0.131438392  \\
            0.102299001  \\
            0.12817915  \\
            0.127195645  \\
            0.11679698  \\
            0.096827718  \\
            0.08834831  \\
            0.076035786  \\
            0.070554223  \\
            0.14293684  \\
            0.129760546  \\
            0.130686645  \\
            0.282278431  \\
        }
        ;
    \nextgroupplot[xlabel={$m = 20$}, ymajorticks={false}, yminorticks={false}]
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.036538022  \\
            0.064586889  \\
            0.048949047  \\
            0.053881499  \\
            0.053767528  \\
            0.048241774  \\
            0.034492873  \\
            0.039946051  \\
            0.043622211  \\
            0.023349395  \\
            0.035118805  \\
            0.038540093  \\
            0.038141928  \\
            0.035146994  \\
            0.03550563  \\
            0.034730579  \\
        }
        ;
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.100915148  \\
            0.095067336  \\
            0.091142703  \\
            0.086381779  \\
            0.065800637  \\
            0.055919843  \\
            0.079796912  \\
            0.088631073  \\
            0.065783393  \\
            0.049581247  \\
            0.099846645  \\
            0.074240902  \\
            0.051281372  \\
            0.060728542  \\
            0.066569305  \\
            0.074889594  \\
        }
        ;
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.147177888  \\
            0.17009801  \\
            0.093579327  \\
            0.3499903  \\
            0.089037223  \\
            0.102004915  \\
            0.135306907  \\
            0.142514018  \\
            0.096699227  \\
            0.124381995  \\
            0.095315706  \\
            0.079216159  \\
            0.097551471  \\
            0.115562854  \\
            0.116272348  \\
            0.066735476  \\
        }
        ;
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.317227479  \\
            0.214376821  \\
            0.158316723  \\
            0.125707844  \\
            0.136402545  \\
            0.081244491  \\
            0.164434961  \\
            0.140175916  \\
            0.166680719  \\
            0.150849098  \\
            0.166790428  \\
            0.373122528  \\
            0.141583938  \\
            0.105953005  \\
            0.157054335  \\
            0.129851296  \\
        }
        ;
    \nextgroupplot[xlabel={$m = 30$}, ymajorticks={false}, yminorticks={false}]
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.05851974  \\
            0.055863293  \\
            0.066132389  \\
            0.063242253  \\
            0.055337226  \\
            0.040183039  \\
            0.048459618  \\
            0.059530841  \\
            0.052631998  \\
            0.039711685  \\
            0.075628322  \\
            0.052276816  \\
            0.048733808  \\
            0.050445178  \\
            0.045089926  \\
            0.044362199  \\
        }
        ;
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.169874443  \\
            0.094198923  \\
            0.12344351  \\
            0.138939215  \\
            0.123673143  \\
            0.120381282  \\
            0.131496117  \\
            0.092976975  \\
            0.108864006  \\
            0.092944474  \\
            0.091717453  \\
            0.091740266  \\
            0.095253114  \\
            0.072278482  \\
            0.069206888  \\
            0.083435863  \\
        }
        ;
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.163541235  \\
            0.176892779  \\
            0.14315659  \\
            0.324291158  \\
            0.093968816  \\
            0.109180589  \\
            0.174313822  \\
            0.127118335  \\
            0.135587314  \\
            0.1373996  \\
            0.105654226  \\
            0.144593353  \\
            0.126640854  \\
            0.134231  \\
            0.357005448  \\
            0.127874837  \\
        }
        ;
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.213625644  \\
            0.380295971  \\
            0.18878957  \\
            0.187535543  \\
            0.19044611  \\
            0.159683956  \\
            0.20459484  \\
            0.144357784  \\
            0.337751151  \\
            0.157387061  \\
            0.196078165  \\
            0.139859248  \\
            0.1303722  \\
            0.162090857  \\
            0.161586229  \\
            0.175576814  \\
        }
        ;
    \nextgroupplot[xlabel={$m = 40$}, ymajorticks={false}, yminorticks={false}]
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.08283913  \\
            0.075907657  \\
            0.067143545  \\
            0.083308687  \\
            0.078159207  \\
            0.06342256  \\
            0.07017169  \\
            0.059223062  \\
            0.071856814  \\
            0.06851817  \\
            0.061084107  \\
            0.069154632  \\
            0.063879857  \\
            0.068603772  \\
            0.063746269  \\
            0.074290794  \\
        }
        ;
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.117082691  \\
            0.331409054  \\
            0.119293282  \\
            0.135100203  \\
            0.109919931  \\
            0.121420945  \\
            0.100289252  \\
            0.112955637  \\
            0.116979567  \\
            0.110938194  \\
            0.098515366  \\
            0.129538125  \\
            0.287887976  \\
            0.126517499  \\
            0.106494913  \\
            0.160758121  \\
        }
        ;
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.160419708  \\
            0.201474581  \\
            0.182500085  \\
            0.236581637  \\
            0.156894211  \\
            0.1451562  \\
            0.367443783  \\
            0.193853642  \\
            0.225908415  \\
            0.114322111  \\
            0.14627596  \\
            0.13854381  \\
            0.146822094  \\
            0.138876805  \\
            0.199815821  \\
            0.129246937  \\
        }
        ;
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.577353724  \\
            0.196164429  \\
            0.25093075  \\
            0.313344456  \\
            0.185070161  \\
            0.202805302  \\
            0.206604765  \\
            0.183740737  \\
            0.226534059  \\
            0.218909709  \\
            0.324514436  \\
            0.202025965  \\
            0.179024025  \\
            0.165340482  \\
            0.190739522  \\
            0.194614197  \\
        }
        ;
    \nextgroupplot[xlabel={$m = 50$}, ymajorticks={false}, yminorticks={false}]
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.103515012  \\
            0.121892316  \\
            0.098906544  \\
            0.101085128  \\
            0.089009467  \\
            0.292620982  \\
            0.102241962  \\
            0.085340781  \\
            0.085225247  \\
            0.089218635  \\
            0.083902769  \\
            0.10929737  \\
            0.097305599  \\
            0.103870836  \\
            0.091324729  \\
            0.083559476  \\
        }
        ;
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.130682834  \\
            0.148654089  \\
            0.151408105  \\
            0.15287003  \\
            0.339032991  \\
            0.112633252  \\
            0.127529471  \\
            0.113497576  \\
            0.115544032  \\
            0.112443734  \\
            0.103893416  \\
            0.144126883  \\
            0.157106255  \\
            0.109982212  \\
            0.149311991  \\
            0.32473494  \\
        }
        ;
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.173301595  \\
            0.193443414  \\
            0.229784347  \\
            0.228507223  \\
            0.182661746  \\
            0.179046045  \\
            0.175834717  \\
            0.206692766  \\
            0.149806616  \\
            0.43917587  \\
            0.159864559  \\
            0.193656248  \\
            0.205892449  \\
            0.178525931  \\
            0.179385403  \\
            0.1511296  \\
        }
        ;
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.276126894  \\
            0.230346782  \\
            0.307048294  \\
            0.506252035  \\
            0.197467445  \\
            0.232620592  \\
            0.258270791  \\
            0.238155757  \\
            0.243419882  \\
            0.262513739  \\
            0.227924817  \\
            0.248845452  \\
            0.466301187  \\
            0.229619393  \\
            0.211860785  \\
            0.23672229  \\
        }
        ;
    \nextgroupplot[xlabel={$m = 60$}, ymajorticks={false}, yminorticks={false}]
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.115639732  \\
            0.114764651  \\
            0.117387113  \\
            0.120985443  \\
            0.115758905  \\
            0.12692632  \\
            0.123959394  \\
            0.325420008  \\
            0.115220969  \\
            0.111429649  \\
            0.108081942  \\
            0.131210616  \\
            0.121681684  \\
            0.11212147  \\
            0.127978905  \\
            0.120474004  \\
        }
        ;
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.162886367  \\
            0.326729483  \\
            0.182807523  \\
            0.182416381  \\
            0.16103888  \\
            0.200190594  \\
            0.130583713  \\
            0.142645385  \\
            0.161293504  \\
            0.180162852  \\
            0.151043266  \\
            0.124625064  \\
            0.333845819  \\
            0.132755885  \\
            0.135728981  \\
            0.132290475  \\
        }
        ;
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.240910145  \\
            0.247139079  \\
            0.303912918  \\
            0.267083124  \\
            0.190810911  \\
            0.427608724  \\
            0.23531549  \\
            0.228777476  \\
            0.184658088  \\
            0.174396275  \\
            0.219579343  \\
            0.220066597  \\
            0.186280157  \\
            0.235900448  \\
            0.259087361  \\
            0.401176705  \\
        }
        ;
    \addplot+[boxplot, mark={*}]
        table[row sep={\\}, y index={0}]
        {
            data  \\
            0.326559974  \\
            0.254857113  \\
            0.253015752  \\
            0.329474357  \\
            0.296782997  \\
            0.283289855  \\
            0.268532504  \\
            0.266804469  \\
            0.490868205  \\
            0.24789634  \\
            0.219389698  \\
            0.274861555  \\
            0.306650086  \\
            0.252252369  \\
            0.225509455  \\
            0.26318604  \\
        }
        ;
\end{groupplot}
\end{tikzpicture}


==> utils/notation_table.tex <==
% !TEX root = root.tex
\begin{table}[t]
    \centering
    % \setlength\tablecolsep{0pt}
    \renewcommand{\arraystretch}{1.5}
    \hspace*{-0.4cm}
    \caption{Notation\label{tab:notation}}
    \begin{tabular*}{\linewidth}{r l@{\extracolsep{\fill}}}
        \toprule
        % Notation \\
       \multicolumn{2}{c}{\textbf{Notation}} \\ % associated with \PCTAPF{} Problem}} \\
       \midrule
        $\numrobots$ & Number of robots in environment \\
        $\numtasks$ & Number of delivery tasks \\
        $\RobotPosition[i]{t} \in \integers^{2}$ & Position of robot $i$ at time $t$ \\
        $\ObjectPosition[j]{t} \in \integers^{2}$ & Position of object $j$ at time $t$ \\
        $P = (\ProjectGraphVertices, \ProjectGraphEdges)$ & Project Graph \\
        % $\TaskSpec[j] = \TaskSpecDef[j], \TaskSpec[j] \in \ProjectGraphVertices$ & Task specification for object $j$ \\
        $\PickupLocation[j]$ & Pick-up location for task $j$ \\
        $\DropoffLocation[j]$ & Drop-off location for task $j$ \\
        $\processtime[j,k]$ & Processing time between tasks $j$ and $k$ \\ 
        $\TaskAssignment[i]$ & Mission of robot $i$ \\
        $\JointMission = (\TaskAssignment[1], \ldots, \TaskAssignment[\numrobots])$ & Joint mission \\
        % $\EligibilityMatrix[i]{j} \in \integers_2^{\numrobots \times \numtasks}$ & Binary eligibility matrix \\
        $\FinalTime = \max_{j} \TaskCompletionTime[j]$ & Project makespan \\
        $\predecessors[j]$ & Predecessors of task $j$ \\
        $\assignment[]{} \in \reals^{(n+m) \times m}$ & Assignment matrix \\
        $\AgentPath[i]=[\RobotPosition[i]{0},\ldots,\RobotPosition[i]{t}]$ & Path of agent $i$ \\
        $\RoutePlan = (\AgentPath[1], \ldots, \AgentPath[\numrobots])$ & Route plan \\
        $\distmatrix[\cdot]{\cdot}$ & Distance between two points in environment \\
        % $\CBSStateConstraint = \CBSStateConstraintDef[\cdot]{\cdot}{\cdot}$ & CBS state constraint \\
        % $\CBSActionConstraint = \CBSActionConstraintDef[\cdot]{\cdot,\cdot}{\cdot}$ & CBS action constraint \\
        $\ProjectSchedule = (\ScheduleVertices, \ScheduleEdges)$ & Project schedule \\
        $\ScheduleNode \in \ScheduleVertices$ & Schedule node \\
        % $\ActiveSet$ & Active set \\
        % $\ClosedSet$ & Closed set \\
        \bottomrule
        \hspace{1pt}
    \end{tabular*}
  \end{table}

